Conformational Landscape of Oxygen-Containing Naphthalene Derivatives

Polycyclic aromatic compounds (PACs) constitute an important class of molecules found in various environments and are considered important pollutants of the Earth's atmosphere. In particular, functionalization of PACs modify the ring aromaticity, which greatly influences the chemical reactivity of these species. In this work we studied several oxygen-containing PACs, relevant to atmospheric chemistry. We investigated the conformational landscape of four naphthalene-derivative molecules -- namely ,1- and 2-hydroxynaphthalene and 1- and 2-naphthaldehyde -- by means of rotational and vibrational spectroscopy supported by quantum chemical calculations. For 1-hydroxynaphthalene and 1-naphthaldehyde, intramolecular hydrogen bonding and steric effects drive the conformational preferences while for 2-hydroxynaphthalene and 2-naphthaldehyde, the charge distributions allow us to understand the conformational landscape. This work not only demonstrates how the localization of the substitution group in the ring influences the conformational relative energies and but also constitutes a step toward a better understanding of the different chemical reactivity of such functionalized PACs.

==> Tables/2NaphthaldehydeTableFreq.tex <==
\begin{table*}%[htbp]
  \centering \footnotesize
  \caption{Calculated far-IR fundamental vibrational modes of $trans$-2-naphthaldehyde and comparison with experimental assignments. Energies are given in \si{\wn} and intensities in \si{\km\per\mol}. \mam{ajout d'une colonne pour indiquer les modes aux freq les plus precises ?}}
    \begin{tabular}{lc rr c rr c rr}
    \toprule
        &  & \multicolumn{2}{c}{B97-1/cc-pVTZ}  && \multicolumn{2}{c}{MP2/cc-pVTZ} && \multicolumn{1}{c}{Hybrid}  &  \multicolumn{1}{c}{Exp.} \\ \cmidrule{3-4}\cmidrule{6-7}
    $\nu$ & sym. & \multicolumn{1}{c}{$E$(harm)} & \multicolumn{1}{c}{$E$(anharm)} && \multicolumn{1}{c}{$E$(harm)} & \multicolumn{1}{c}{$I$(harm)} && \multicolumn{1}{c}{$E$} &     \\
    \midrule
    32 & A'  & 639 & 633 && 632 & 1.9  && 625 & \\
    33 & A'  & 612 & 606 && 608 & 3.6  && 602 & 603\\
    34 & A'  & 519 & 514 && 516 & 0.1  && 510 & \\
    35 & A'  & 390 & 388 && 385 & 5.5  && 383 & 388\\
    36 & A'  & 348 & 350 && 347 & 2.8  && 348 & \\
    37 & A'  & 176 & 184 && 175 & 6.0  && 182 & 177\\
    47 & A'' & 645 & 639 && 619 & 0.9  && 614 & \\
    48 & A'' & 512 & 507 && 501 & 0.3  && 496 & \\
    49 & A'' & 485 & 479 && 476 & 15.9 && 471 &  472   \\
    50 & A'' & 400 & 395 && 392 & 0.04 && 387 & \\
    51 & A'' & 297 & 289 && 293 & 3.3  && 285 & \\
    52 & A'' & 191 & 187 && 187 & 4.7  && 183 & 181   \\
    53 & A'' & 160 & 156 && 156 & 4.8  && 152 & 152   \\
    54 & A'' & 78  & 77  && 77  & 1.6  && 75  & \\          
    \bottomrule
    \end{tabular}%
      \label{tab:trans2NaphthalVibFreq}%
\end{table*}%



==> Tables/DeltaQ.tex <==
\begin{table}[htbp]
  \centering \footnotesize
  \caption{Calculated global charge re-distribution upon functionalization, $\Delta Q$ (unitless). See text and eq. \ref{eqDQ} for details.}
    \begin{tabular}{l c}
    \toprule
    species$^a$	&	$\Delta Q^b$ 	\\ \midrule
    1-naphthaldehyde	&	5.36	\\
    2-naphthaldehyde	&	4.99	\\
    \\
    1-hydroxynaphthalene &	7.14	\\
    2-hydroxynaphthalene	&	7.22	\\
    \bottomrule
    \end{tabular}
    
    \medskip
    \begin{minipage}{0.45 \textwidth}
    $^a$ Only the most stable conformer of each species is considered.\\
    $^b$ see text and eq. \ref{eqDQ}.
    \end{minipage}
    
      \label{tab:DQ}%
\end{table}%
